Quick-Draw Bandits: Quickly Optimizing in Nonstationary Environments with Extremely Many Arms

Canonical algorithms for multi-armed bandits typically assume a stationary reward environment where the size of the action space (number of arms) is small. More recently developed methods typically relax only one of these assumptions: existing non-stationary bandit policies are designed for a small number of arms, while Lipschitz, linear, and Gaussian process bandit policies are designed to handle a large (or infinite) number of arms in stationary reward environments under constraints on the reward function. In this manuscript, we propose a novel policy to learn reward environments over a continuous space using Gaussian interpolation. We show that our method efficiently learns continuous Lipschitz reward functions with $\mathcal{O}^*(\sqrt{T})$ cumulative regret. Furthermore, our method naturally extends to non-stationary problems with a simple modification. We finally demonstrate that our method is computationally favorable (100-10000x faster) and experimentally outperforms sliding Gaussian process policies on datasets with non-stationarity and an extremely large number of arms.

==> theory/notation.tex <==
\begin{table}[t]
    \caption{Math notation table}
    \begin{tabular}{ll}
    \toprule
    Symbol & Meaning \\
    \midrule
    $\mathcal{X}$   &    the set of arms, located within a compact metric space \\
    $K$   &   number of arms (discrete setting) \\
    $\mathcal{S}$   &   a subset of arms in $\mathcal{X}$ \\
    $T$     &     time horizon of bandit sampling \\
    $\mu(x, t)$    &    mean payout at arm $x\in \mathcal{X}$ and time $t$ \\
    $y(x, t)$   &   the observed payout at arm $x$ at time $t$ \\
    $\mathcal{R}(x, t)$   &  instantaneous regret of arm $x$ at time $t$   \\
    $\mathcal{R}_T$   &    cumulative regret over $T$ rounds \\
    $\rho^2$   &    observation variance of each arm \\
    $L$  & Lipschitz constant of observation function \\
    $\tau_s$; $\tau_e$   &   respective time intervals between observations; reward environment change \\
    $D(\cdot, \cdot)$  &  distance metric over $\mathcal{X}$ \\
    $\mathcal{D}_i$ &  notates an observed payout $y(x_i, t_i)$ within a sequence \\
    $\mathcal{P}$ & probability density or mass function \\
    $d$   & dimension of $\mathcal{X}$ \\
    \bottomrule
    \end{tabular}
\end{table}

